Partial Quantifier Elimination By Certificate Clauses

In this report, we study partial quantifier elimination (PQE) for propositional CNF formulas. PQE is a generalization of quantifier elimination where one can limit the set of clauses taken out of the scope of quantifiers to a small subset of target clauses. The appeal of PQE is twofold. First, PQE can be dramatically simpler than full quantifier elimination. Second, PQE provides a language for performing incremental computations. Many verification problems (e.g. equivalence checking and model checking) are inherently incremental and so can be solved in terms of PQE. Our approach is based on deriving clauses depending only on unquantified variables that make the target clauses $\mathit{redundant}$. Proving redundancy of a target clause is done by construction of a "certificate" clause implying the former. We describe a PQE algorithm called $\mathit{START}$ that employs the approach above. To evaluate $\mathit{START}$, we apply it to invariant generation for a sequential circuit $N$. The goal of invariant generation is to find an $\mathit{unwanted}$ invariant of $N$ proving unreachability of a state that is supposed to be reachable. If $N$ has an unwanted invariant, it is buggy. Our experiments with FIFO buffers and HWMCC-13 benchmarks suggest that $\mathit{START}$ can be used for detecting bugs that are hard to find by existing methods.

==> c5ert_der_exmp.tex <==
\section{Derivation Of Certificate When A Conflict Occurs (An Example)}
\label{app:cert_der}



==> junk.tex <==

\vspace{20pt}

%just something to fill out the page
\clearpage
just something to fill out the page
\clearpage


==> storage.tex <==
The last version of this report was published in May, 2022.
--
Subsection~\ref{ssec:triv} presents a procedure for identifying target
clauses that are trivially redundant.
---
In formulas generated off circuits trivial redundancy occurs quite
often.
------
If, when proving proving redundancy of the new copy
of $C$, \Apqe takes a different path, generation of a duplicate does
not lead to \ti{looping}.  However, sometimes \Apqe does loop even on
small formulas.
---------
There are two reasons for \Apqe to generate duplicate participant
certificates.  First, \Apqe processes one target clause at a
time. (So, for instance, \apqe that proves redundancy redundancy of
all target clauses together does not loop.) Second, when a conflict
clause containing quantified variables is added to the formula it may
become a new target clause that needs to proved redundant in a some
subspace.
%
To address the first reason, one can just relax the requirement to
process only one target clause at a time. For instance, if a duplicate
of a target clause $C$ earlier proved redundant is generated when
proving redundancy of $C'$, it makes sense to prove the redundancy of
$C$ and $C'$ \ti{together}. So, instead of choosing between two
extreme paradigms of either processing all clauses together (\apqe) or
one clause at a time (\Apqe), one can consider joing processing of a
\ti{subset} of target clauses. The second reason for generating
duplicate certificates can be addessed by avoiding adding conflict
clauses with quantified variables. However, this requires a radical
overhaul of the current approach to PQE solving.
-----------
(Below, we omit the modifier
``participant. So, when we say ``certificate'' we mean
``\ti{participant} certificate''.)
---------
In~\cite{cert_tech_rep} we introduced the notion of a certificate
clause that can be viewed as an advanced form of a D-sequent.  The
idea here is to prove a clause $C$ redundant in subspace \pnt{q} by
deriving a clause $K$ that \ti{implies} $C$ in subspace \pnt{q}.  The
clause $K$ is called a certificate.
----------
The predecessor of the approach based on certificate clauses is the
machinery of dependency sequents
(D-sequents)~\cite{fmcad12,fmcad13}. A D-sequent is a record stating
redundancy of a clause in a quantified formula. A flaw of this
machinery is that to reuse a learned D-sequent, one has to keep a lot
of contextual information~\cite{qe_learn}, which makes D-sequent
reusing expensive.  On the other hand, the reuse of certificate
clauses does not require to store any contextual information.
-------
In this section, we cast a retrospective look at \Apqe in the light
of some new results obtained recently.
----
Interpolation~\cite{craig,ken03} is also a special case
of PQE~\cite{tech_rep_pc_lor}.
----------
(A
mature PQE algorithm can be applied to a long list of problems
including those listed in Section~\ref{sec:using_pqe}.)
--------
In
Sections~\ref{sec:inv_gen}-\ref{sec:exper1}, we use \Apqe for
invaraint generation.
--------
Ideally, we
would like to apply \Apqe to a known problem e.g. one listed in
Section~\ref{sec:using_pqe} and compare it with existing tools.
However, PQE-solving is still in its infancy and must go through many
improvements before it matures. (PQE is much more complex than, say,
SAT. As mentioned above, SAT is a special case of QE and QE is a
special case of PQE.)
----------
Section~\ref{sec:interp}
shows that interpolation is a special case of PQE.  In
Section~\ref{sec:using_pqe}, to demonstrate the versatility of PQE, we
recall reductions of a few well known problems to PQE.

